From Trees to Gravity

In this article we study two related models of quantum geometry: generic random trees and two-dimensional causal triangulations. The Hausdorff and spectral dimensions that arise in these models are calculated and their relationship with the structure of the underlying random geometry is explored. Modifications due to interactions with matter fields are also briefly discussed. The approach to the subject is that of classical statistical mechanics and most of the tools come from probability and graph theory.

==> T2G New Archive version/totalmacroe.tex <==
%\documentclass[10pt]{article}
%\usepackage{color} %used for font color
%\usepackage{amssymb} %maths
%\usepackage{amsmath} %maths
%\usepackage[utf8]{inputenc} %useful to type directly diacritic characters
%\begin{document}
%\input{Bbb}

\newcommand{\rf}[1]{(\ref{#1})}
\newcommand{\oh}{\frac{1}{2}}
\newcommand{\oq}{\frac{1}{4}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\beas}{\begin{eqnarray*}}
\newcommand{\eeas}{\end{eqnarray*}}
\newcommand{\beqs}{\begin{displaymath}}
\newcommand{\eeqs}{\end{displaymath}}
\newcommand{\ra}{\rightarrow}
%slash (gn bogstav, 2 variationer: \fsll=lowercase, \fslu=uppercase letters)
\newcommand{\fslu}{\not\mbox{\hspace{-1.5mm}}}   
\newcommand{\fsll}{\not\mbox{\hspace{-.5mm}}}   
\newcommand{\br}{\langle}
\newcommand{\kt}{\rangle}
% \kt højre kommando = >
\newcommand{\bra}[1]{\langle {#1}|}
% <...| \bra{...} {... fx vector i}
\newcommand{\ket}[1]{|{#1}\rangle}
\newcommand{\ul}{\underline}
\newcommand{\dg}{\dagger}
\newcommand{\5}{5 \! \times \! 5}
\newcommand{\nn}{\nonumber \\}
%---------------------------------------
\newcommand{\ab}{abelian}
\newcommand{\ch}{chirality}
\newcommand{\Cou}{Coulomb}
\newcommand{\Gf}{Green functions}
\newcommand{\Fm}{Feynman}
\newcommand{\ham}{hamiltonian}
\newcommand{\lag}{lagrangian}
\newcommand{\Lo}{Lorentz}
\newcommand{\Mi}{Minkowski}
\newcommand{\mi}{minkowskian}
\newcommand{\Eu}{Euclid}
\newcommand{\eu}{euclidean}
\newcommand{\WT}{Ward-Takahashi}
\newcommand{\sm}{standard model}
%---------------------------
%\renewcommand{\pt}{\partial}
\renewcommand{\a}{\alpha}
\renewcommand{\b}{\beta}
\newcommand{\g}{\gamma}
\newcommand{\G}{\Gamma}
\newcommand{\del}{\delta}
\newcommand{\Del}{\Delta}
\newcommand{\ep}{\varepsilon}
\newcommand{\e}{\epsilon}
\newcommand{\ka}{\kappa}
\newcommand{\kp}{\kappa}
%\renewcommand{\l}{\lambda}
%\renewcommand{\L}{\Lambda}
\newcommand{\m}{\mu}
\newcommand{\vmu}{\vec{\mu}}
\newcommand{\n}{\nu}
\newcommand{\mn}{\mu\nu} 
\newcommand{\om}{\omega}
\newcommand{\vom}{\vec{\omega}}
\newcommand{\tphi}{\tilde{\phi}}
\newcommand{\phid}{\phi^{\dagger}}
\newcommand{\ff}{\phi^3}
\newcommand{\fF}{\phi^4}
\newcommand{\fn}{\phi^n}
\newcommand{\bpsi}{\bar{\psi}}
\newcommand{\rh}{\rho}
\newcommand{\sg}{\sigma}
\newcommand{\vsig}{\vec{\sigma}}
\newcommand{\Sg}{\Sigma}
%\newcommand{\th}{\theta}
%\newcommand{\Th}{\Theta}
\newcommand{\vp}{\varphi}
%----------------------------------
%\renewcommand{\thepage}{}
%---------------------------------
\newcommand{\vB}{\vec{B}}
\newcommand{\cD}{{\cal D}}

\newcommand{\cH}{{\cal H}}

\newcommand{\uN}{\underline{N}}
\newcommand{\uM}{\underline{M}}


\newcommand{\be}{\bar{e}}
%\newcomand{\te}{\tilde{e}}
\newcommand{\bl}{\bar{\l}}
\newcommand{\cL}{{\cal L}}
\newcommand{\vL}{\vec{L}}
\newcommand{\cE}{{\cal E}}
\newcommand{\cM}{{\cal M}}
\newcommand{\cG}{{\cal G}}
\newcommand{\cP}{{\cal P}}   
\newcommand{\cB}{{\cal B}}
\newcommand{\cT}{{\cal T} }
\newcommand{\cO}{{\cal O}}
\newcommand{\vS}{\vec{S}}
\newcommand{\cV}{{\cal V}}
\newcommand{\hk}{\hat{k}}
\newcommand{\vk}{\vec{k}}
\newcommand{\vek}{\vec{k}\mbox{\hspace{1mm}}}
\newcommand{\hq}{\hat{q}}
\newcommand{\vx}{\vec{x}}
\newcommand{\vex}{\vec{x}\mbox{\hspace{1mm}}}
\newcommand{\hr}{\hat{r}}
\newcommand{\Tr}{{\rm Tr}\;}
%----------------------------------------
%Jens macro commands
%----------------------------------------
\newcommand{\ben}{\begin{equation}}
\newcommand{\een}{\end{equation}}

%\newcommand{\bea}{\begin{eqnarray}}
%\newcommand{\eea}{\end{eqnarray}}
\newcommand{\bdm}{\begin{displaymath}}
\newcommand{\edm}{\end{displaymath}}
%\newcommand{\nn}{\nonumber \\ }
\newcommand{\hf}{\frac{1}{2}}
%\newcommand{\vx}{\vec{x}}
%\newcommand{\vk}{\vec{k}}
\newcommand{\vn}{\vec{\nabla}}
\newcommand{\ve}{\vec{e}}
\newcommand{\vep}{\vec{e}\mbox{\hspace{1mm}}'}
\newcommand{\La}{{\cal L}}
\newcommand{\Ha}{{\cal H}}
\newcommand{\pa}{\partial}
%\newcommand{\del}{\delta}
\newcommand{\eps}{\epsilon}
\newcommand{\al}{\alpha}
%\newcommand{\fslu}{\not\mbox{\hspace{-1.5mm}}}   
%\newcommand{\fsll}{\not\mbox{\hspace{-.5mm}}}   
%\newcommand{\D}{{\cal D}}
\newcommand{\N}{{\cal N}}
\newcommand{\tb}{\overline{t}}
\newcommand{\qh}{\hat{q}}
\newcommand{\phih}{\hat{\phi}}
%\newcommand{\g}{\gamma}
%\newcommand{\G}{\Gamma}
\newcommand{\gb}{\overline{\gamma}}
\newcommand{\zt}{\zeta}
\newcommand{\ztb}{\overline{\zeta}}
\newcommand{\tq}{\tilde{q}}
%\newcommand{\br}{\langle}
%\newcommand{\kt}{\rangle}
%\newcommand{\bra}[1]{\langle {#1}|}
%\newcommand{\ket}[1]{|{#1}\rangle}
\newcommand{\Asf}{{\sf A}}
\newcommand{\Bsf}{{\sf B}}
\newcommand{\Csf}{{\sf C}}
\newcommand{\ps}{\psi}
\newcommand{\psb}{\overline{\psi}}
\newcommand{\etb}{\overline{\eta}}
\newcommand{\Phc}{\Phi^{Cl}}
%-------------------------------------------------
%---- chiral chapter
\renewcommand{\d}{\delta}
\newcommand{\cJ}{{\cal J}}
\newcommand{\vph}{\varphi}

\renewcommand{\dag}{\dagger}
\newcommand{\tr}{{\rm tr}\,}
\newcommand{\lla}{\left\langle}
\newcommand{\rra}{\right\rangle}
\newcommand{\DS}{\!\!\!\! /}
\newcommand{\ds}{\!\!\!\! \hspace{1mm} /}

\newcommand{\bbN}{\mathbb N}
\newcommand{\bbZ}{{\mathbb Z}}
\newcommand{\bbR}{{\mathbb R}}
\newcommand{\bbC}{{\mathbb C}}
\newcommand{\bbQ}{{\mathbb Q}}
\newcommand{\bbP}{{\mathbb P}}

\newcommand{\bon}{{\bf n}}

